Multi-hop Question Answering under Temporal Knowledge Editing

Multi-hop question answering (MQA) under knowledge editing (KE) has garnered significant attention in the era of large language models. However, existing models for MQA under KE exhibit poor performance when dealing with questions containing explicit temporal contexts. To address this limitation, we propose a novel framework, namely TEMPoral knowLEdge augmented Multi-hop Question Answering (TEMPLE-MQA). Unlike previous methods, TEMPLE-MQA first constructs a time-aware graph (TAG) to store edit knowledge in a structured manner. Then, through our proposed inference path, structural retrieval, and joint reasoning stages, TEMPLE-MQA effectively discerns temporal contexts within the question query. Experiments on benchmark datasets demonstrate that TEMPLE-MQA significantly outperforms baseline models. Additionally, we contribute a new dataset, namely TKEMQA, which serves as the inaugural benchmark tailored specifically for MQA with temporal scopes.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section/2_Introduction.tex <==
\section{Introduction}
\label{sec:intro}
\vspace{-0.1in}
Large Language Models (LLMs) have received widespread attention due to their immense abilities to comprehend knowledge, offering tailored solutions for a wide range of applications \citep{Zhao2023ASO,Huang2022TowardsRI}. However, outdated knowledge limits the abilities of LLMs to provide accurate responses about recent events and facts, a phenomenon known as hallucinations, where LLMs tend to fabricate plausible yet incorrect responses about unknown facts \citep{Hong2023FaithfulQA}. Thus, it is vitally important to keep the LLMs updated with the latest available information. However, as the most direct approach for updating information, editing LLMs by re-training from scratch is practically infeasible, as it requires huge computational resources and substantial investments. 
For this, \textit{Knowledge Editing} (KE), which aims to precisely modify/update the knowledge in LLMs without retraining the model, has thus received much attention in recent years \citep{2023_KE_Survey,Zhang2024ACS}. 


Multi-hop question answering (MQA), on the other hand, aims to answer complex questions requiring multiple reasoning steps. For MQA, KE entails \textit{``ripple effects''}, i.e., a single edit may trigger a series/chain of knowledge edits/updates \citep{Cohen2023EvaluatingTR}. For instance, if we update the knowledge about the U.S. president from \textit{Trump} to \textit{Biden}, correspondingly knowledge for the question: ``Who is the wife of the U.S. president?'' should also be updated \citep{Cohen2023EvaluatingTR}. There are two prominent lines of work in this area: parameter-based editing and memory-based editing. %with the latter outperforming the former in most of the cases.
The parameter-based editing methods update the knowledge by directly modifying the parameters of the model \citep{meng2022locating,meng2022mass}, while memory-based methods maintain an explicit memory to store information about the facts to be modified \citep{Mitchell2022MemoryBasedME,zhong2023mquake,gu2023pokemqa}. In most cases, the memory-based approaches 
outperform the parameter-based methods \citep{gu2023pokemqa,zhong2023mquake}


To address ripple effects, memory-based methods adapt plan-and-solve paradigm \citep{Khot2022DecomposedPA, Wang2023PlanandSolvePI}, where LLMs are prompted to decompose multi-hop questions into sub-questions, followed by iteratively answering each sub-question. 
To find relevant edits for each sub-question, they use dense retrieval to compare the semantic similarity for each sub-question \citep{Karpukhin2020DensePR}. However, we observed that these approaches exhibit a key limitation, i.e., they perform poorly on questions with explicit temporal contexts \citep{Yin2023HistoryMT}. This inability to cater to temporal context is attributed to the dense retrieval employed by the memory-based methods, which primarily store the edit retrieval information in an unstructured format. This is illustrated in Figure~\ref{fig:challenge} (a), where the dense retrieval retrieves an irrelevant fact (from the year 2022) for the question {\em ``Who was the owner of Tom's company in 2020?''}.


.................\warn{Fill this GAP}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{Figure/Fig1.pdf}
    \caption{\textbf{Limitations of dense retrieval to handle temporal context.} 
    (a) There is a temporal constraint in question. However, this temporal information is not correctly captured by dense retrieval, thus yielding an erroneous retrieval.
    (b) The time-aware graph stores edits as a time-conscious knowledge structure to help distinguish temporal context and improve retrieval accuracy.}
    \vspace{-3.7ex}
    \label{fig:challenge}
\end{figure}


To address the aforementioned limitations, we propose a method called~\OurMODEL{}: \underline{\textbf{TEMP}}oral know\underline{\textbf{LE}}dge augmented \underline{\textbf{M}}ulti-hop \underline{\textbf{Q}}uestion \underline{\textbf{A}}nswering. \OurMODEL{} first constructs a time-aware graph (TAG) to store the edit information in a structured format to preserve the context-specific temporal information in the best possible way (Figure~\ref{fig:challenge} (b)).%\fixchen{Why Graph in Figure~\ref{fig:challenge}(b) is different from graph in Figure~\ref{fig:Vs}}
In order to improve the retrieval performance across semantically related edits, \OurMODEL{}: (i) uses data augmentation techniques to capture the alias for entity names helpful for entity disambiguation, (ii) uses context-dependent concepts to explicitly filter the edits based on 
contextual similarity. In order to solve the multi-hop questions, \OurMODEL{} uses pre-trained LLMs to come up with an inference path and perform step-by-step joint reasoning by utilizing the LLMs and TAG to come up with the final response. Experimental evaluation using benchmark data sets 
shows that~\OurMODEL{} outperforms the existing state-of-the-art work on MQA by a significant margin. We summarize the key contributions of this work as follows. 

\begin{itemize}
    \item We propose~\OurMODEL{}, the first method capable of achieving high accuracy on MQA  under a large amount of temporal knowledge edit without forgetting historical knowledge. 
    \item Unlike previous approaches, \OurMODEL{} constructs a TAG to store structured information via our developed methods. Moreover, we propose a new planning procedure and a joint reasoning approach for the inference path, and we develop a novel structural retrieval procedure for retrieving knowledge, which can be used for other problems. 
    \item Extensive experimental results on two benchmark datasets show that \OurMODEL{} outperforms the previous five baselines via different metrics for MQA under massive edits. Moreover, we developed a new dataset, namely MQAuKE, which could be considered the first benchmark on multi-hop questions with temporal scopes. 
\end{itemize}



%%%%%%%%%%%%% EXTRA-STUFF %%%%%%%%%%%%%%%


\eat{
While in most cases, \eat{recent studies show that }the memory-based approaches 
outperform the parameter-based methods ~\cite{gu2023pokemqa,zhong2023mquake}, 
we observe these existing solutions still pose the following \eat{key }limitations:
(i) these methods perform poorly on questions with explicit temporal contexts,
(ii) their performance degrades for mass-edit scenarios. 
\eat{\di{reference}.} } 


%\warn{This causes \di{this is caused by, or this is the reason?} some useful historical knowledge to be forgotten during knowledge updating.}


%\textbf{(ii) The mass edit} problem implies that a large number of semantically related edits stored in the edit memory make it difficult for the dense retrieval to find the correct edit. This in turn significantly degrades the overall performance of the end model.For instance, Zhong et al.,~\cite{zhong2023mquake} highlighted that the accuracy of MeLLo declines by 37.2\% when the number of edits is increased beyond 3,000. \fixchen{How about adjust the story line and focus on designing a multi-key retrieval for memory-based method and temporal edit.}




%For performance evaluation, we used an MQA benchmark dataset,  i.e., \textsc{MQuAKE} by Zhong et al.,~\cite{zhong2023mquake}.  To further test the abilities of~\OurMODEL{} for mass-edit settings  and a wide variations of temporal contexts, we also introduce an evaluation benchmark \OurDataset{}: \underline{\textbf{T}}emporal \underline{\textbf{K}}nowledge \underline{\textbf{E}}diting on \underline{\textbf{M}}ulti-hop \underline{\textbf{Q}}uestion \underline{\textbf{A}}nswering. keeping in view the limitations of \textsc{MQuAKE} (discussed in details in Appendix~\ref{appendix:limitations}). Experimentation evaluation shows that~\OurMODEL{} greatly surpasses  existing methods, achieving state-of-the-art performance. \fixchen{Report some percentage improvement here...!} 


%\warn{Specifically, \OurMODEL{} convert edit memory to time-conscious knowledge graphs, which store edits in four dimensions in the aforementioned structured way. It uses Wikidata for data augmentation to find all the aliases for entities to address name entity ambiguous. \OurMODEL{} uses structural retrieval which perform the four points stated above. The sub-question also need to be structured similar to edit, thus \OurMODEL{} extracts the inference path for multi-hop question, which is a sequence of triplet.}


\eat{\OurMODEL{} employs time conscious knowledge graph to stores edits, helpful 
to augment the retrieval performance of the model.} 


\eat{In order to overcome the challenges such as: aliases for entities,} 

\eat{Also, it caters to the lexical variations of semantically related relation, e.g., ``live in'' and ``reside in'', \OurMODEL{} use dense retrieval to compare semantic relevance to distinguish them.}


\eat{\warn{It uses Wikidata for data augmentation to find all the aliases for entities to address ambiguous name entity . 
Moreover, \OurMODEL{} leverages our proposed planning and joint reasoning for a novel structure retrieval to retrieve knowledge for editing.} }

\eat{In order to overcome the challenges such as: aliases for entities, e.g., {"Donald Trump" vs "Donald J. Trump"}, \OurMODEL{} uses wikidata to conduct data augmentation to find all the aliases for entities.}

\eat{The \eat{former changes}\asif{parameter-based editing methods update the} knowledge by modifying the parameters of the model. 
The latter stores \asif{information about facts} in an explicit memory 
without modifying the parameters of the model\eat{and performs better in this task}~\cite{Mitchell2022MemoryBasedME,zhong2023mquake,gu2023pokemqa}.} 


\eat{We also observe deficiencies in the \textsc{MQuAKE} benchmark and propose a new knowledge editing dataset incorporating temporal retrieval and mass-editing challenges.
1) There are conflicts between edits. Some edits are modified in some questions and not modified in some questions. 2) The alias of the answer is not enough. 3) The generated multi-hop question misses sub-questions.}

\eat{
In order to augment 
the retrieval performance across multiple different contexts, it uses structural 
retrieval to retrieve the edit along four different dimensions}


\eat{Our crucial observation for the above limitation is that \textbf{previous work overlooks the importance of the structural nature of knowledge for retrieval.} Generally speaking, each piece of knowledge can be structured into four dimensions: subject, relation, object, and time, e.g., <Twitter, owner is, Elon Musk, 2022, N/A> \di{Ok, now I know the structure, but why previous work overlook it?}.
Independently analyzing the four dimensions we can get possible directions for improving the retrieval: 1) Determine whether the edit's subject is the same as the subject of sub-question. However, there is name entity ambiguous issue: Subject may have many aliases, e.g., "Donald Trump" vs "Donald J. Trump" \di{I do not know what your main idea, you want to say analyzing each dimension can improve the performance, but here you mention there are some issues.}. 2) Explicitly store the validity period of each edit and compare it with the query time interval. 3) For a given context subject entity type tells about person, org, loc etc helps in dis-ambigiuation. e.g., "Trump tower" vs "Trump" \di{What does this mean?}. 4) Lexical variation: there are semantically similar relations, e.g., “live in” and “reside in”, use dense retrieval to distinguish them. Previous work only solved the fourth point, thus leading to the above limitation. \di{I do not understand what you want to say and your main idea, try to rewrite it.} }


\eat{However, as shown in Figure~\ref{fig:challenge}-b, using time conscious 
knowledge graph to explicitly store the time information in a structured 
form helps the model to circumvent this problem significantly.}





\eat{To address the aforementioned limitations, we propose a method called~\OurMODEL{}: Multi-hop Question Answering under Temporal Knowledge Editing. 
\OurMODEL{} first constructs a time-aware graph (TAG) to store the 
edit information in a structured format to preserve the context-specific 
temporal information in the best possible way (Figure~\ref{fig:challenge}-b).\fixchen{Why Graph in Figure~\ref{fig:challenge}(b) is different
from graph in Figure~\ref{fig:Vs}}
In order to improve the retrieval performance across semantically related 
edits, \OurMODEL{}: (i) uses data augmentation techniques to capture the alias for entity names helpful for entity disambiguation, 
(ii) uses context-dependent concepts to explicitly filter the edits based on 
contextual similarity. 
In order to solve the multi-hop questions, \OurMODEL{} uses pre-trained 
LLMs to come up with an inference path and performs a step-by-step 
joint reasoning by utilizing the LLMs and TAG to come up with the 
final response.}

==> section/XXTRA_Approach2.tex <==
\section{Edit Database}
In this section, we introduce the edit database $\mathcal{D}$ used by \textsc{RwEF}. This database $\mathcal{D}$ is divided into four dimensions to store fact edits $\mathcal{E}$ , and employ a retrieval $\mathbf{R_{edit}}$ to use different retrieve rule in each dimension. Specifically, the retrieval $\mathbf{R_{edit}}$ can be divided into two steps: 1) Filter: Filter out the edits that do not meet the required subject and time limit. 2) Rerank: Rerank remaining edits based on semantic similarity.
%Due to the non-uniqueness of reasoning paths and the existence of skipping phenomena, we need a broader span of editing, where the span refers to the combination of multiple relations. We maintain a knowledge editing graph $G_{editing}$, where each node can serve as a subject or object, and each edge is a directed edge with a specific relation. If some datasets represent editing in the form of natural language sequence. We need to convert the editing $e_i$ into a triplet form $(s_i, r_i,o_i)$. For two connected editings in the graph, we can obtain a combined editing between them based on transitivity. In the ideal scenario, we could compute the transitive closure of $G_{editing}$, but this would introduce significant retrieval overhead.

%With the increasing number of edits, accurately identifying the corresponding editing poses a challenge. The previous sub-question decomposition method retrieves the editing directly from the sub-question, in which performance is not optimal. One reason is that the sub-problem has a different form from editing, while we standardize the sub-problem and editing into the same $(s,r,o)$ format. Another reason is that they encode editing in the form of complete natural language sequences, whereas we design rules based on three different dimensions $s,r,o$ for retrieval.

\subsection{Edit Database}
Previous work ignore the structure of edit, resulting in low retrieval performance. The retrieval $\mathbf{R_{edit}}:(s_i,r_i,o_i^\prime,t) \rightarrow edit,sim$ aims to find the most relevant edit in $\mathcal{D}$. That is to say, we need to find the edit where corresponding to subject entity $s_i$, the relation is $r_i$, the modification time is less than $t$, and the object type is $o$. Specifically, $\mathbf{R_{edit}}$ retrieve according to the following two steps: 

\textbf{Step1 Filter based on subject and time.} $\mathbf{R_{edit}}$ initially employed the subject $s$ and time $t$ dimension for filtering, identifying edits $e$, in which $e[s]$ is identical to the subject $s_i$ of the key and $e[t]$ is less than the time $t$. 
\begin{equation}
   \mathcal{D}_{sub} = \{e\mid e \in \mathcal{D} \ \& \ e[s] = s_i \ \& \ e[t]<t\}
    \label{eq:Re1}
\end{equation}
where $\mathcal{D}_{sub}$ is the remaining edits.\\
\\
\textbf{Step2 Rerank based on relation and object.} Then, $\mathbf{R_{edit}}$ retrieve based the relation $r$ and object $o$ dimensions. $\mathbf{R_{edit}}$ employ an encoder to get the vector embedding $v_{q}$ and $V_{editing}$ of the key and remaining edits $\mathcal{D}_{sub}$:
\begin{equation}
   v_{q}=Encoder(s_i\oplus r_i \oplus o_i^\prime)
    \label{eq:Ret1}
\end{equation}
\begin{equation}
   V_{edits}=\{Encoder(e[s]\oplus e[r] \oplus Type(e[o]))\mid e \in \mathcal{D}_{sub}\}
    \label{eq:Ret2}
\end{equation}
Where $Type(e.o)$ denotes the type of editing object $e.o$. We use cosine similarity to measure the similarity between vectors, selecting the highest similarity as the retrieval result.
\begin{equation}
    e_{result},cosine(v_{result},v_q) = \argmax_{e_i,v_i \in \mathcal{D}_{sub},V_{edits}} {\frac{v_q \cdot v_i}{\lVert v_q \rVert \lVert v_i \rVert}}
    \label{eq:Ret3}
\end{equation} 
where $e_{result}$ is the most relevant edit, and $cosine(v_{result},v_q)$ is the similarity between the key and this edit $e_{result}$.


